MoCaE: Mixture of Calibrated Experts Significantly Improves Object Detection

Combining the strengths of many existing predictors to obtain a Mixture of Experts which is superior to its individual components is an effective way to improve the performance without having to develop new architectures or train a model from scratch. However, surprisingly, we find that na\"ively combining expert object detectors in a similar way to Deep Ensembles, can often lead to degraded performance. We identify that the primary cause of this issue is that the predictions of the experts do not match their performance, a term referred to as miscalibration. Consequently, the most confident detector dominates the final predictions, preventing the mixture from leveraging all the predictions from the experts appropriately. To address this, when constructing the Mixture of Experts, we propose to combine their predictions in a manner which reflects the individual performance of the experts; an objective we achieve by first calibrating the predictions before filtering and refining them. We term this approach the Mixture of Calibrated Experts and demonstrate its effectiveness through extensive experiments on 5 different detection tasks using a variety of detectors, showing that it: (i) improves object detectors on COCO and instance segmentation methods on LVIS by up to $\sim 2.5$ AP; (ii) reaches state-of-the-art on COCO test-dev with $65.1$ AP and on DOTA with $82.62$ $\mathrm{AP_{50}}$; (iii) outperforms single models consistently on recent detection tasks such as Open Vocabulary Object Detection.

==> Sections/1.Introduction_old.tex <==
\section{Introduction}\label{sec:introduction}
Visual detection requires each object in the image to be localised and classified.
%
\blockcomment{
\begin{table}
    \small
    %\setlength{\tabcolsep}{0.45em}
    \centering
    \caption{Oracle Performance. Calibrated: The score of the bounding box matches with IoU of the ground truth box that the box has the most overlap with. }
    \label{tab:oracle}
    \scalebox{1.0}{
    \begin{tabular}{c|c||c|c|c||c|c|c||c|c|c|} 
    \toprule
    \midrule
    Detector & Calibrated?&AP&AP50&AP75&APS&APM&APL&ECE-eq. w.&ECE&MCE   \\ \midrule
    F-RCNN&uncalibrated&$40.1$&$60.8$&$44.0$&$26.0$&$44.3$&$51.9$&$10.62$&$0.22$&$24.47$\\
    F-RCNN&LR&$39.7$&$60.5$&$43.5$&$25.9$&$44.31$&$51.2$&$9.07$&$0.08$&$21.15$\\
    F-RCNN&IR&$39.8$&$60.4$&$43.5$&$26.0$&$43.9$&$51.4$&$5.32$&$0.03$&$25.33$\\
    F-RCNN&oracle&$74.7$&$91.6$&$83.0$&$60.4$&$80.2$&$88.0$&$0.00$&$0.00$&$0.00$\\ \midrule
    RS R-CNN&uncalibrated& $42.4$&$62.1$&$46.3$&$26.8$&$46.3$&$56.9$&$18.93$&$13.79$&$35.37$\\
    RS R-CNN&LR& $26.4$&$36.9$&$29.1$&$13.6$&$28.0$&$40.7$&$25.68$&$0.44$&$61.11$ \\
    RS R-CNN&IR& $41.9$&$61.6$&$46.0$&$26.6$&$46.0$&$56.0$&$5.12$&$0.03$&$22.80$\\
    RS R-CNN&oracle& $75.4$&$92.2$&$82.6$&$60.4$&$81.2$&$90.2$&$0.00$&$0.00$& $0.00$\\\midrule
    ATSS&uncalibrated&$43.1$&$61.5$&$47.1$&$27.9$&$47.5$&$54.3$&&\\ 
    ATSS&oracle&$77.3$&$92.3$&$84.6$&$61.7$&$84.5$&$90.1$&&\\ \midrule
    PAA&uncalibrated&$43.3$&$60.8$&$47.1$&$27.0$&$47.0$&$57.6$&&\\ 
    PAA&oracle&$78.9$&$92.6$&$85.3$&$63.2$&$85.9$&$92.8$&&\\ 
    \midrule
    \bottomrule
    \end{tabular}
    }
\end{table}
}

Depending on the need of the application, the object is localized by different representations each of which is generally framed by a different type of detection problem in the literature.
%
Object detection uses axis-aligned bounding boxes, instance segmentation localises the objects with masks in pixel-level, keypoint detection uses a set of keypoints for localisation and rotated object detection allows different orientation of bounding boxes as well.
%
The models devised for such visual detection tasks are critical components of the perception systems, and their safe and reliable usage requires their outputs to be calibrated, which has not received a significant attention in the community. 
%
In this paper, we present a comprehensive guide on the calibration of visual detectors to address this limitation in the literature.

Existing definitions of calibration focused on the specific problem of object detection and other critical visual detection tasks such as instance segmentation have been ignored.
%
Furthermore, broadly speaking, the existing definitions of calibration on object detection either consider classification calibration or localisation calibration, ignoring the fact that object detection is a joint problem of these two tasks.
%
As an example, Detection ECE considers precision but not the localisation quality and it is class-agnostic.
%
Differently, Oksuz et al. introduce Localisation-aware ECE that requires the confidence of the detections to be aligned with the product of precision and average IoU representing classification and localisation performance respectively.
%
Furthermore, following how AP is computed, LaECE is first computed class-wise and then it is averaged.
%
While this perspective addresses an important gap, this might not be necessarily the case how accuracy is defined in the target application.
%
To illustrate, an application may require a different localisation error than IoU, which is in the case of LVIS instance segmentation benchmark relying on Boundary IoU.
%
Furthermore, while an application can put equal importance to both performance aspects, some may not; or some applications might require the performance to be class-agnostic, for others long-tail classes might be important.
%
Existing definitions are not generic to address the needs of such applications.

Current evaluation of calibration error in object detection is also conducted on the expected calibration error.
%
There are several metrics in the classification and localisation calibration which may be preferable to the expected calibration error...

In this paper, we focus on the calibration of visual detectors from a more \textbf{general} perspective in two aspects: First, we define Generalized Localisation-aware Calibration by following a generic definition of visual detection task. 
%
Therefore, our definition of calibration can be adopted by different visual detection tasks.
%
Second, considering Generalized Localization-aware Calibration we define Expected, Maximum, Average Localization-aware calibration errors as well as Quality Focal Loss to measure the calibration error.
%
While being na\"ive extensions, we believe that these calibration errors will play an important part in developing more robust object detectors.

Furthermore, we mainly focus on the calibration of visual detectors from a \textbf{practical} perspective. 
%
Namely, we investigate why calibrating object detectors is important in practice, which is also ignored by the literature.
%
This investigation led us to identify that the calibration is crucial for visual detectors in two levels, both of which correspond to the special cases of our generalized definition: 
%
\begin{itemize}
    \item Model calibration refers to the calibration of the raw probabilities, which are consumed by the post-processing steps in visual detectors,
    \item Detector calibration corresponds to the calibration of final probabilities after the postprocessing, which are then propagated to the downstream task. 
\end{itemize}
%
\begin{figure}[t]
        \centering
        \includegraphics[width=0.98\textwidth]{example-image}
        \caption{Teaser to demonstrate benefit of calibration to obtain proper mixture of experts.
        }
        \label{fig:teaser}
\end{figure} 
We identify three critical benefits of model calibration in visual detectors: We first show that the model calibration decreases the sensitivity of the hyperparameters of the models in postprocessing, which directly affect the efficiency and accuracy of the detector.
%
From a broader perspective, this level of calibration facilitates decoupling the model from the postprocessing pipeline.
%
Thereby enabling the practitioners to modify or replace their models without paying significant attention to the postprocessing to preserve efficiency or accuracy.
%
% can easily standardize postprocessing efficiency across different detectors and allow more accurate postprocessing modules to be incorporated into the detection pipeline. 
%
Secondly, model calibration enables us to obtain more accurate mixture of experts using different types of detectors. 
%
While the individual models are miscalibrated, the most overconfident model, though possibly the least accurate, dominates the output of the mixture of experts and results in significantly lower accuracy.
%
We show that once model calibrated, the resulting MoE consistently outperforms its individual detectors by a notable margin in different tasks and datasets.
%
%We believe that this can promote different mixture of experts type approaches for visual detection tasks, which are missing in the literature.
%
And third, long-tail classes, which are conventionally suppressed by the detector \cite{Norcal}, are promoted through calibration.
%
Finally, we focus on detector calibration and provide a guide on how to derive a proper calibration definition as well as the associated errors in various use-cases based on our generalized Localisation-aware calibration.

Our contributions can be summarized as follows:
\begin{itemize}
    \item We define Generalized Localization-aware Calibration for visual detection tasks. Based on this definition, we derive different types (maximum, expected, average etc.) of localisation-aware calibration errors.
    \item We split calibration in visual detectors in two-levels. More specifically, we introduce Model Calibration and show that it is useful for abstracting away postprocessing from the model, obtaining a proper mixture of experts and improving long-tail recognition. And for Detector Calibration, we discuss how to design a calibration criterion and metrics based on our general perspective.
    \item We show that isotonic regression is a competitive baseline for both of these calibration levels. Considering the highly imbalanced nature of Model Calibration, a na\"ive class-wise implementation of post-hoc calibration methods decreases the performance. We fix this by leveraging the methods from the imbalance literature.
\end{itemize}





\blockcomment{

\begin{table}
    \small
    \setlength{\tabcolsep}{0.25em}
    \centering
    \caption{No ensemble is proper AP(ensemble) $\geq$ max(AP(model1),...,AP(modelN)) without calibration.}
    \label{tab:ensemble}
    \scalebox{1.0}{
    \begin{tabular}{c|c|c|c|c||c|c|c||c|c|c||c|c|c} 
    \toprule
    \midrule
    Calibration&F-RCNN&RS-RCNN&ATSS&PAA&AP&AP50&AP75&APS&APM&APL&ECE&MCE&ACE \\ \midrule
    None&\cmark& & & &$40.1$&$60.8$&$44.0$&$26.0$&$44.3$&$51.9$&$0.22$&$24.47$&$10.62$\\
    Class-wise LR&\cmark&&& &$39.7$&$60.5$&$43.5$&$25.9$&$44.1$&$51.2$&$0.09$&$21.15$&$9.07$\\
    %Class-wise IR&\cmark& & & &$39.8$&$60.4$&$43.5$&$26.0$&$43.9$&$51.4$&$0.03$&$24.92$&$5.30$\\
    Class-wise IR&\cmark& & & &$39.8$&$60.4$&$43.6$&$26.0$&$43.8$&$51.4$&$0.03$&$25.20$&$5.33$\\
    Class-agnostic LR&\cmark& & & &$40.2$&$60.8$&$44.0$&$26.0$&$44.3$&$51.9$&$0.20$&$23.40$&$9.87$\\   
    %Class-agnostic IR&\cmark& & & &$40.3$&$61.3$&$44.0$&$26.7$&$44.4$&$52.1$&$0.14$&$14.87$&$6.04$\\ 
    Class-agnostic IR&\cmark& & & &$40.3$&$61.3$&$44.0$&$26.7$&$44.4$&$52.1$&$0.14$&$14.82$&$6.05$\\
    \midrule

    None&&\cmark& & &$42.4$&$62.1$&$46.3$&$26.8$&$46.3$&$56.9$&$13.79$&$35.37$&$5.18$\\
    Class-wise LR&&\cmark& & &$26.4$&$36.9$&$29.1$&$13.6$&$28.0$&$40.7$&$0.44$&$61.11$&$25.12$\\
    %Class-wise IR& &\cmark& & &$41.9$&$61.6$&$46.0$&$26.6$&$46.0$&$56.0$&$0.03$&$23.90$&$5.18$\\
    Class-wise IR& &\cmark& & &$41.9$&$61.5$&$46.0$&$26.6$&$46.0$&$56.1$&$0.03$&$25.10$&$5.23$\\
    Class-agnostic LR& &\cmark& & &$42.4$&$62.1$&$46.3$&$26.8$&$46.3$&$56.9$&$0.65$&$68.81$&$27.48$\\
    %Class-agnostic IR&&\cmark& & &$42.4$&$62.1$&$46.3$&$26.7$&$46.3$&$56.7$&$0.13$&$14.07$&$5.86$\\
    Class-agnostic IR&&\cmark& & &$42.4$&$62.2$&$46.4$&$26.8$&$46.3$&$56.7$&$0.14$&$14.08$&$5.86$\\
    \midrule

    
    None&&&\cmark& &$43.1$&$61.5$&$47.1$&$27.9$&$47.5$&$54.3$&$0.20$&$42.53$&$25.22$\\
    Class-wise LR&&&\cmark& &$42.0$&$60.4$&$45.9$&$27.4$&$46.5$&$52.4$&$0.12$&$24.79$&$10.13$\\
    %Class-wise IR& & &\cmark& &$41.9$&$61.6$&$46.0$&$26.6$&$46.0$&$56.0$&$0.02$&$25.37$&$5.45$\\
    Class-wise IR& & &\cmark& &$42.8$&$60.9$&$46.6$&$28.4$&$47.2$&$54.1$&$0.02$&$25.38$&$5.40$\\
    Class-agnostic LR& & &\cmark& &$42.8$&$61.5$&$46.8$&$27.8$&$47.3$&$53.8$&$0.17
    $&$23.07$&$7.86$\\
    %Class-agnostic IR&&&\cmark & &$43.1$&$61.5$&$47.1$&$28.0$&$47.4$&$54.3$&$0.15$&$15.52$&$7.09$\\
    Class-agnostic IR&&&\cmark & &$43.1$&$61.6$&$47.1$&$28.0$&$47.5$&$54.4$&$0.10$&$15.59$&$6.43$\\
    \midrule

%PAA

    None&&&&\cmark &$43.3$&$60.8$&$47.1$&$27.0$&$47.0$&$57.6$&$3.39$&$19.80$&$9.73$\\
    Class-wise LR&&&&\cmark &$37.1$&$50.9$&$40.6$&$19.1$&$40.6$&$53.2$&$0.22$&$60.05$&$28.95$\\
    %Class-wise IR& & &&\cmark &$42.5$&$59.8$&$46.4$&$25.9$&$46.4$&$56.4$&$0.03$&$26.30$&$5.24$\\
    Class-wise IR& & &&\cmark &$42.5$&$59.8$&$46.4$&$25.9$&$46.4$&$56.6$&$0.03$&$26.60$&$5.26$\\
    Class-agnostic LR& & &&\cmark &$43.3$&$60.8$&$47.1$&$27.0$&$47.0$&$57.6$&$0.37
    $&$54.03$&$25.49$\\
    %Class-agnostic IR&&& &\cmark &$43.2$&$60.8$&$47.1$&$27.4$&$47.0$&$57.6$&$0.19$&$18.08$&$7.23$\\
    Class-agnostic IR&&& &\cmark &$43.2$&$60.8$&$47.1$&$27.4$&$47.0$&$57.6$&$0.19$&$18.08$&$7.23$\\
    \midrule
    \bottomrule
    \end{tabular}
    }
\end{table}



\begin{table}
    \small
    \setlength{\tabcolsep}{0.25em}
    \centering
    \caption{No ensemble is proper AP(ensemble) $\geq$ max(AP(model1),...,AP(modelN)) without calibration.}
    \label{tab:ensemble}
    \scalebox{1.0}{
    \begin{tabular}{c|c|c|c|c||c|c|c||c|c|c||c|c|c} 
    \toprule
    \midrule
    Calibration&F-RCNN&RS-RCNN&ATSS&PAA&AP&AP50&AP75&APS&APM&APL&ECE&MCE&ACE \\ \midrule
    %\multirow{4}{*}{None}&\cmark& & & %&$39.9$&$60.9$&$43.6$&$24.9$&$43.7$&$49.8$\\
    %&& \cmark& & &$42.0$&$62.2$&$45.7$&$25.7$&$45.6$&$55.0$ & & &\\
    %&& & \cmark&  &$42.8$&$61.3$&$46.6$&$27.3$&$47.0$&$53.0$& & &\\ 
    %&& & &  \cmark&$43.1$&$60.9$&$46.6$&$26.7$&$46.9$&$56.0$& & &\\ \midrule
    %\multirow{4}{*}{None}&\cmark&\cmark & & &$40.8$&$61.1$&$45.2$&$25.9$&$44.8$&$51.5$& & &\\
    %&\cmark& &\cmark & &$40.6$&$61.0$&$44.9$&$26.2$&$44.6$&$50.1$& & &\\
    %&\cmark& & &\cmark &$41.1$&$61.6$&$45.4$&$26.8$&$45.0$&$51.6$& & &\\
    %&\cmark&\cmark&\cmark& \cmark&$41.0$&$61.2$&$45.4$&$26.2$&$45.0$&$51.7$& & & \\
    %\bottomrule
    None&\cmark& & & &$40.1$&$60.8$&$44.0$&$26.0$&$44.3$&$51.9$&$0.22$&$24.47$&$10.62$\\
    None - Soft NMS, $\sigma=0.50$&\cmark& & & &$40.6$&$61.3$&$44.8$&$26.7$&$44.5$&$52.4$&$0.22$&$24.47$&$10.62$\\
    Class-wise LR&\cmark&&& &$39.7$&$60.5$&$43.5$&$25.9$&$44.1$&$51.2$&$0.09$&$21.15$&$9.07$\\
    %Class-wise IR&\cmark& & & &$39.8$&$60.4$&$43.5$&$26.0$&$43.9$&$51.4$&$0.03$&$24.92$&$5.30$\\
    Class-wise IR&\cmark& & & &$39.8$&$60.4$&$43.6$&$26.0$&$43.8$&$51.4$&$0.03$&$25.20$&$5.33$\\
    Class-agnostic LR&\cmark& & & &$40.2$&$60.8$&$44.0$&$26.0$&$44.3$&$51.9$&$0.20$&$23.40$&$9.87$\\   
    %Class-agnostic IR&\cmark& & & &$40.3$&$61.3$&$44.0$&$26.7$&$44.4$&$52.1$&$0.14$&$14.87$&$6.04$\\ 
    Class-agnostic IR&\cmark& & & &$40.3$&$61.3$&$44.0$&$26.7$&$44.4$&$52.1$&$0.14$&$14.82$&$6.05$\\
    Class-agnostic IR - Soft NMS, $\sigma=1.00$&\cmark& & & &$40.8$&$60.7$&$44.9$&$27.0$&$44.9$&$52.7$&$0.14$&$14.82$&$6.05$\\
    \midrule

    None&&\cmark& & &$42.4$&$62.1$&$46.3$&$26.8$&$46.3$&$56.9$&$13.79$&$35.37$&$5.18$\\
    None - Soft NMS, $\sigma=0.50$&&\cmark& & &$41.5$&$60.7$&$45.5$&$25.9$&$45.5$&$55.8$&$13.79$&$35.37$&$5.18$\\
    Class-wise LR&&\cmark& & &$26.4$&$36.9$&$29.1$&$13.6$&$28.0$&$40.7$&$0.44$&$61.11$&$25.12$\\
    %Class-wise IR& &\cmark& & &$41.9$&$61.6$&$46.0$&$26.6$&$46.0$&$56.0$&$0.03$&$23.90$&$5.18$\\
    Class-wise IR& &\cmark& & &$41.9$&$61.5$&$46.0$&$26.6$&$46.0$&$56.1$&$0.03$&$25.10$&$5.23$\\
    Class-agnostic LR& &\cmark& & &$42.4$&$62.1$&$46.3$&$26.8$&$46.3$&$56.9$&$0.65$&$68.81$&$27.48$\\
    %Class-agnostic IR&&\cmark& & &$42.4$&$62.1$&$46.3$&$26.7$&$46.3$&$56.7$&$0.13$&$14.07$&$5.86$\\
    Class-agnostic IR&&\cmark& & &$42.4$&$62.2$&$46.4$&$26.8$&$46.3$&$56.7$&$0.14$&$14.08$&$5.86$\\
    Class-agnostic IR  - Soft NMS, $\sigma=1.00$ &&\cmark& & &$42.8$&$61.6$&$47.4$&$26.9$&$46.8$&$57.4$&$0.14$&$14.08$&$5.86$\\
    \midrule

    
    None&&&\cmark& &$43.1$&$61.5$&$47.1$&$27.9$&$47.5$&$54.3$&$0.20$&$42.53$&$25.22$\\
    None - Soft NMS, $\sigma=0.50$&&&\cmark& &$42.9$&$61.7$&$46.7$&$28.5$&$47.1$&$54.0$&$0.20$&$42.53$&$25.22$\\
    Class-wise LR&&&\cmark& &$42.0$&$60.4$&$45.9$&$27.4$&$46.5$&$52.4$&$0.12$&$24.79$&$10.13$\\
    %Class-wise IR& & &\cmark& &$41.9$&$61.6$&$46.0$&$26.6$&$46.0$&$56.0$&$0.02$&$25.37$&$5.45$\\
    Class-wise IR& & &\cmark& &$42.8$&$60.9$&$46.6$&$28.4$&$47.2$&$54.1$&$0.02$&$25.38$&$5.40$\\
    Class-agnostic LR& & &\cmark& &$42.8$&$61.5$&$46.8$&$27.8$&$47.3$&$53.8$&$0.17
    $&$23.07$&$7.86$\\
    %Class-agnostic IR&&&\cmark & &$43.1$&$61.5$&$47.1$&$28.0$&$47.4$&$54.3$&$0.15$&$15.52$&$7.09$\\
    Class-agnostic IR&&&\cmark & &$43.1$&$61.6$&$47.1$&$28.0$&$47.5$&$54.4$&$0.14$&$15.22$&$6.79$\\
    Class-agnostic IR - Soft NMS, $\sigma=1.00$ &&&\cmark & &$43.2$&$61.8$&$47.2$&$28.8$&$47.4$&$54.6$&$0.14$&$15.22$&$6.79$\\
    \midrule

%PAA

    None&&&&\cmark &$43.3$&$60.8$&$47.1$&$27.0$&$47.0$&$57.6$&$3.39$&$19.80$&$9.73$\\
    None - Soft NMS, $\sigma=0.50$&&&&\cmark &$42.4$&$60.3$&$45.9$&$26.2$&$45.7$&$56.7$&$3.39$&$19.80$&$9.73$\\
    Class-wise LR&&&&\cmark &$37.1$&$50.9$&$40.6$&$19.1$&$40.6$&$53.2$&$0.22$&$60.05$&$28.95$\\
    %Class-wise IR& & &&\cmark &$42.5$&$59.8$&$46.4$&$25.9$&$46.4$&$56.4$&$0.03$&$26.30$&$5.24$\\
    Class-wise IR& & &&\cmark &$42.5$&$59.8$&$46.4$&$25.9$&$46.4$&$56.6$&$0.03$&$26.60$&$5.26$\\
    Class-agnostic LR& & &&\cmark &$43.3$&$60.8$&$47.1$&$27.0$&$47.0$&$57.6$&$0.37
    $&$54.03$&$25.49$\\
    %Class-agnostic IR&&& &\cmark &$43.2$&$60.8$&$47.1$&$27.4$&$47.0$&$57.6$&$0.19$&$18.08$&$7.23$\\
    Class-agnostic IR&&& &\cmark &$43.2$&$60.8$&$47.1$&$27.4$&$47.0$&$57.6$&$0.19$&$18.08$&$7.23$\\
    Class-agnostic IR - Soft NMS, $\sigma=1.00$ &&& &\cmark &$43.3$&$60.8$&$47.1$&$27.1$&$46.8$&$57.9$&$0.19$&$18.08$&$7.23$\\
    
    \midrule
    
    None&\cmark&\cmark & & &$41.1$&$62.0$&$45.1$&$27.1$&$45.0$&$53.8$& & &\\
    Class-wise LR&\cmark&\cmark & & &$39.4$&$60.0$&$43.4$&$25.9$&$43.7$&$51.2$& & &\\
    %Class-wise IR&\cmark&\cmark & & &$42.0$&$62.1$&$46.0$&$27.4$&$46.0$&$55.3$& & &\\
    Class-wise IR&\cmark&\cmark & & &$42.0$&$62.1$&$46.0$&$27.4$&$46.0$&$55.3$& & &\\
    Class-agnostic LR&\cmark&\cmark & & &$40.6$&$61.5$&$44.4$&$27.0$&$44.6$&$52.3$& & &\\
    %Class-agnostic IR&\cmark&\cmark & & &$42.6$&$62.7$&$46.5$&$27.7$&$46.4$&$56.4$& & &\\
    Class-agnostic IR&\cmark&\cmark & & &$42.6$&$62.7$&$46.5$&$27.7$&$46.4$&$56.4$& & &\\
    Class-agnostic IR  - Soft NMS, $\sigma=1.00$&\cmark&\cmark & & &$43.1$&$62.4$&$47.6$&$28.0$&$47.0$&$56.8$& & &\\
    \midrule
    
    None (NMS=0.5)&&\cmark &\cmark& &$42.4$&$62.1$&$46.3$&$26.8$&$46.3$&$56.9$& & &\\
    None (NMS=0.6)&&\cmark &\cmark& &$42.4$&$61.3$&$46.7$&$26.8$&$46.5$&$56.7$& & &\\
    Class-agnostic LR (NMS=0.5)&&\cmark &\cmark& &$42.7$&$62.1$&$46.2$&$28.6$&$47.1$&$53.5$& & &\\
    Class-agnostic IR (NMS=0.5)&&\cmark &\cmark& &$43.9$&$63.5$&$47.8$&$28.7$&$47.9$&$56.8$& & &\\
    Class-agnostic IR (NMS=0.6)&&\cmark &\cmark& &$43.9$&$62.7$&$48.4$&$28.7$&$48.2$&$56.8$& & &\\
    Class-agnostic IR  - Soft NMS, $\sigma=1.00$&&\cmark &\cmark& &$44.3$&$63.2$&$48.8$&$29.6$&$48.3$&$57.4$& & &\\
    %Class-agnostic IR (NMS=0.5)&&\cmark &\cmark& &$43.9$&$63.5$&$47.8$&$28.7$&$47.9$&$56.9$& & &\\
%    \bottomrule
%    None (NMS=0.5)&\cmark&\cmark &\cmark& &$41.1$&$62.0$&$45.1$&$27.1$&$45.0$&$53.8$& & &\\
%    Class-agnostic LR (NMS=0.5)&\cmark&\cmark &\cmark& &$42.5$&$62.8$&$45.9$&$28.4$&$46.8$&$54.3$& & &\\
%    Class-agnostic IR (NMS=0.5)&\cmark&\cmark &\cmark& &$43.8$&$63.5$&$47.7$&$29.0$&$47.7$&$56.5$& & &\\
    %Class-agnostic IR (NMS=0.6)&\cmark&\cmark &\cmark& &$43.8$&$63.5$&$47.7$&$28.9$&$47.7$&$56.6$& & &\\
    \bottomrule
    None (NMS=0.5)&\cmark&\cmark &\cmark&\cmark&$41.3$&$61.3$&$45.9$&$27.4$&$45.5$&$53.9$& & &\\
    Class-agnostic LR (NMS=0.5)&\cmark&\cmark &\cmark&\cmark&$42.6$&$62.0$&$46.6$&$28.5$&$47.2$&$54.5$& & &\\
    %Class-agnostic IR (NMS=0.5)&\cmark&\cmark &\cmark&\cmark&$44.5$&$62.9$&$48.9$&$29.5$&$48.8$&$57.8$& & &\\
    Class-agnostic IR (NMS=0.5)&\cmark&\cmark &\cmark&\cmark&$44.5$&$63.8$&$48.3$&$29.5$&$48.5$&$57.6$& & &\\
    Class-agnostic IR - Soft NMS, $\sigma=1.00$&\cmark&\cmark &\cmark&\cmark&$44.8$&$63.7$&$49.1$&$29.6$&$48.8$&$58.3$& & &\\
    \bottomrule
    \end{tabular}
    }
\end{table}

\begin{table}
    \small
    \setlength{\tabcolsep}{0.25em}
    \centering
    \caption{SAOD-Gen ID Test Set}
    \label{tab:ensemble}
    \scalebox{1.0}{
    \begin{tabular}{c|c|c|c||c|c|c||c|c|c|} 
    \toprule
    \midrule
    Calibration&RS-RCNN&ATSS&PAA&AP&AP50&AP75&APS&APM&APL \\ \midrule
    None&\cmark& & &$28.6$&$41.2$&$31.2$&$10.5$&$25.8$&$40.1$\\ \midrule
    None&&\cmark& &$28.8$&$39.9$&$31.2$&$10.6$&$26.6$&$39.7$\\ \midrule
    % None (NMS=0.5)&\cmark &\cmark& &$42.4$&$62.1$&$46.3$&$26.8$&$46.3$&$56.9$\\
    Class-agnostic IR (on minival 2500 images)&\cmark &\cmark& &$29.5$&$41.7$&$32.2$&$11.3$&$27.0$&$40.8$\\
    %Class-agnostic IR (on val 5000 images)&\cmark &\cmark& &$29.5$&$41.5$&$32.2$&$11.2$&$26.9$&$41.5$\\
    Class-agnostic IR  - Soft NMS, $\sigma=1.00$&\cmark &\cmark& &$29.6$&$41.3$&$32.6$&$11.3$&$27.1$&$40.9$\\
    \bottomrule
    \end{tabular}
    }
\end{table}



\begin{table}
    \small
    \setlength{\tabcolsep}{0.45em}
    \centering
    \caption{NMS inefficiency due to improper background removal. All times are in ms}
    \label{tab:nmsineff}
    \scalebox{1.0}{
    \begin{tabular}{c||c|c|c|c|c|c|c|c|} 
    \toprule
    \midrule
    &\multicolumn{4}{|c|}{CUDA-NMS}&\multicolumn{4}{|c|}{Pytorch-NMS}   \\ \midrule
    Detector&AP&Inf time&NMS time&Model time&AP&Inf time&NMS time&Model time   \\ \midrule
    F-RCNN&$39.9$&$67.5$&$0.5$&$67.0$&$39.8$&$82.4$&$15.5$&$66.9$\\
    RS-RCNN &$42.0$&$101.4$&$35.4$&$66.0$&$?$&$6375.5$&$6308.6$&$66.9$\\
    ATSS &$42.8$&$60.2$&$0.6$&$59.6$&$42.7$&$46.0$&$105.6$&$59.6$\\
    PAA &$43.1$&$88.2$&$29.2$&$59.0$&$43.1$&$3149.2$&$3091.7$&$57.5$\\
    \bottomrule
    \end{tabular}
    }
\end{table}

\begin{table}
    \small
    \setlength{\tabcolsep}{0.25em}
    \centering
    \caption{No ensemble is proper AP(ensemble) $\geq$ max(AP(model1),...,AP(modelN)) without calibration. Need to fix that None are on entire val set.}
    \label{tab:ensemble1}
    \scalebox{1.0}{
    \begin{tabular}{c|c|c|c|c||c|c|c||c|c|c||c|c|c} 
    \toprule
    \midrule
    Calibration&F-RCNN&RS-RCNN&ATSS&PAA&AP&AP50&AP75&APS&APM&APL&ECE&MCE&ACE \\ \midrule
    None&\cmark& & & &$40.1$&$60.8$&$44.0$&$26.0$&$44.3$&$51.9$&$0.07$&$26.27$&$10.81$\\
    Class-wise LR&\cmark&&& &$39.7$&$60.5$&$43.5$&$25.9$&$44.1$&$51.2$&$0.05$&$18.91$&$7.08$\\
    %Class-wise IR&\cmark& & & &$39.8$&$60.4$&$43.5$&$26.0$&$43.9$&$51.4$&$0.03$&$24.92$&$5.30$\\
    Class-wise IR&\cmark& & & &$39.8$&$60.4$&$43.6$&$26.0$&$43.8$&$51.4$&$0.01$&$30.68$&$6.21$\\
    Class-agnostic LR&\cmark& & & &$40.2$&$60.8$&$44.0$&$26.0$&$44.3$&$51.9$&$0.08$&$21.02$&$8.12$\\   
    %Class-agnostic IR&\cmark& & & &$40.3$&$61.3$&$44.0$&$26.7$&$44.4$&$52.1$&$0.14$&$14.87$&$6.04$\\ 
    Class-agnostic IR&\cmark& & & &$40.3$&$61.3$&$44.0$&$26.7$&$44.4$&$52.1$&$0.06$&$16.97$&$6.40$\\ 
    \midrule

    % RS RCNN

    None&&\cmark& & &$42.4$&$62.1$&$46.3$&$26.8$&$46.3$&$56.9$&$13.93$&$39.56$&$20.82$\\
    Class-wise LR&&\cmark& & &$26.4$&$36.9$&$29.1$&$13.6$&$28.0$&$40.7$&$0.35$&$53.44$&$23.76$\\
    %Class-wise IR& &\cmark& & &$41.9$&$61.6$&$46.0$&$26.6$&$46.0$&$56.0$&$0.03$&$23.90$&$5.18$\\
    Class-wise IR& &\cmark& & &$41.9$&$61.5$&$46.0$&$26.6$&$46.0$&$56.1$&$0.01$&$29.56$&$6.15$\\
    Class-agnostic LR& &\cmark& & &$42.4$&$62.1$&$46.3$&$26.8$&$46.3$&$56.9$&$0.49$&$57.52$&$22.62$\\
    %Class-agnostic IR&&\cmark& & &$42.4$&$62.1$&$46.3$&$26.7$&$46.3$&$56.7$&$0.13$&$14.07$&$5.86$\\
    Class-agnostic IR&&\cmark& & &$42.4$&$62.2$&$46.4$&$26.8$&$46.3$&$56.7$&$0.06$&$15.97$&$6.29$\\
    \midrule

    
    None&&&\cmark& &$43.1$&$61.5$&$47.1$&$27.9$&$47.5$&$54.3$&$0.24$&$41.65$&$22.92$\\
    Class-wise LR&&&\cmark& &$42.0$&$60.4$&$45.9$&$27.4$&$46.5$&$52.4$&$0.11$&$32.59$&$15.24$\\
    %Class-wise IR& & &\cmark& &$41.9$&$61.6$&$46.0$&$26.6$&$46.0$&$56.0$&$0.02$&$25.37$&$5.45$\\
    Class-wise IR& & &\cmark& &$42.8$&$60.9$&$46.6$&$28.4$&$47.2$&$54.1$&$0.00$&$32.02$&$5.99$\\
    Class-agnostic LR& & &\cmark& &$42.8$&$61.5$&$46.8$&$27.8$&$47.3$&$53.8$&$0.14
    $&$26.83$&$10.93$\\
    %Class-agnostic IR&&&\cmark & &$43.1$&$61.5$&$47.1$&$28.0$&$47.4$&$54.3$&$0.15$&$15.52$&$7.09$\\
    Class-agnostic IR&&&\cmark & &$43.1$&$61.6$&$47.1$&$28.0$&$47.5$&$54.4$&$0.03$&$17.89$&$7.61$\\\midrule

%PAA

    None&&&&\cmark &$43.3$&$60.8$&$47.1$&$27.0$&$47.0$&$57.6$&$3.52$&$22.72$&$11.11$\\
    Class-wise LR&&&&\cmark &$37.1$&$50.9$&$40.6$&$19.1$&$40.6$&$53.2$&$0.19$&$64.69$&$30.69$\\
    %Class-wise IR& & &&\cmark &$42.5$&$59.8$&$46.4$&$25.9$&$46.4$&$56.4$&$0.03$&$26.30$&$5.24$\\
    Class-wise IR& & &&\cmark &$42.5$&$59.8$&$46.4$&$25.9$&$46.4$&$56.6$&$0.01$&$33.67$&$6.24$\\
    Class-agnostic LR& & &&\cmark &$43.3$&$60.8$&$47.1$&$27.0$&$47.0$&$57.6$&$0.28
    $&$62.85$&$28.83$\\
    %Class-agnostic IR&&& &\cmark &$43.2$&$60.8$&$47.1$&$27.4$&$47.0$&$57.6$&$0.19$&$18.08$&$7.23$\\
    Class-agnostic IR&&& &\cmark &$43.2$&$60.8$&$47.1$&$27.4$&$47.0$&$57.6$&$0.08$&$20.84$&$7.86$\\\midrule
    
    None&\cmark&\cmark & & &$41.1$&$62.0$&$45.1$&$27.1$&$45.0$&$53.8$& & &\\
    Class-wise LR&\cmark&\cmark & & &$39.4$&$60.0$&$43.4$&$25.9$&$43.7$&$51.2$& & &\\
    %Class-wise IR&\cmark&\cmark & & &$42.0$&$62.1$&$46.0$&$27.4$&$46.0$&$55.3$& & &\\
    Class-wise IR&\cmark&\cmark & & &$42.0$&$62.1$&$46.0$&$27.4$&$46.0$&$55.3$& & &\\
    Class-agnostic LR&\cmark&\cmark & & &$40.6$&$61.5$&$44.4$&$27.0$&$44.6$&$52.3$& & &\\
    %Class-agnostic IR&\cmark&\cmark & & &$42.6$&$62.7$&$46.5$&$27.7$&$46.4$&$56.4$& & &\\
    Class-agnostic IR&\cmark&\cmark & & &$42.6$&$62.7$&$46.5$&$27.7$&$46.4$&$56.4$& & &\\
    \midrule
    
    None (NMS=0.5)&&\cmark &\cmark& &$42.4$&$62.1$&$46.3$&$26.8$&$46.3$&$56.9$& & &\\
    None (NMS=0.6)&&\cmark &\cmark& &$42.4$&$61.3$&$46.7$&$26.8$&$46.5$&$56.7$& & &\\
    Class-agnostic LR (NMS=0.5)&&\cmark &\cmark& &$42.7$&$62.1$&$46.2$&$28.6$&$47.1$&$53.5$& & &\\
    Class-agnostic IR (NMS=0.5)&&\cmark &\cmark& &$43.9$&$63.5$&$47.8$&$28.7$&$47.9$&$56.8$& & &\\
    Class-agnostic IR (NMS=0.6)&&\cmark &\cmark& &$43.9$&$62.7$&$48.4$&$28.7$&$48.2$&$56.8$& & &\\
    %Class-agnostic IR (NMS=0.5)&&\cmark &\cmark& &$43.9$&$63.5$&$47.8$&$28.7$&$47.9$&$56.9$& & &\\
    \bottomrule
    None (NMS=0.5)&\cmark&\cmark &\cmark& &$41.1$&$62.0$&$45.1$&$27.1$&$45.0$&$53.8$& & &\\
    Class-agnostic LR (NMS=0.5)&\cmark&\cmark &\cmark& &$42.5$&$62.8$&$45.9$&$28.4$&$46.8$&$54.3$& & &\\
    Class-agnostic IR (NMS=0.5)&\cmark&\cmark &\cmark& &$43.8$&$63.5$&$47.8$&$28.9$&$47.8$&$56.4$& & &+\\
    %Class-agnostic IR (NMS=0.6)&\cmark&\cmark &\cmark& &$43.8$&$63.5$&$47.7$&$28.9$&$47.7$&$56.6$& & &\\
    \bottomrule
    None (NMS=0.5)&\cmark&\cmark &\cmark&\cmark&$41.3$&$61.3$&$45.9$&$27.4$&$45.5$&$53.9$& & &\\
    Class-agnostic LR (NMS=0.5)&\cmark&\cmark &\cmark&\cmark&$42.6$&$62.0$&$46.6$&$28.5$&$47.2$&$54.5$& & &\\
    %Class-agnostic IR (NMS=0.5)&\cmark&\cmark &\cmark&\cmark&$44.5$&$62.9$&$48.9$&$29.5$&$48.8$&$57.8$& & &\\
    Class-agnostic IR (NMS=0.5)&\cmark&\cmark &\cmark&\cmark&$44.5$&$63.8$&$48.4$&$29.4$&$48.6$&$57.5$& & &+\\
    \bottomrule
    \end{tabular}
    }
\end{table}

Earlier work proposed some metrics but they do not investigate why it is important to calibrate object detectors.

Main research questions of the paper: At what levels do we need calibration for object detectors? Why do we need them? How should we calibrate? 

Main Hypotheses of the paper:
\begin{itemize}
    \item \textit{Hypothesis 1: Calibration enables the detectors to be abstracted away from both the postprocessing and the downstream tasks:} 
    The literature heavily focuses on improving the Average Precision measure. However, as discussed by the earlier work, AP is not generally aligned with the requirement of the downstream tasks such as prediction or surveillance. As a result, the modifications in the detection pipeline (such as replacing the existing detector by a stronger one or training the existing detector for the sake of improving AP) do not simply imply a gain in terms of the efficiency of the detector or the downstream task accuracy without tailoring the hyper-parameters for each of the modifications. Here, we identify that the underlying factors of this performance drop are two fold: 
    \begin{itemize}
        \item Factor 1: The distribution shift of the NMS scores originating from different detectors as well as the different design choices for the same detector affects the efficiency of the detector. To demonstrate this, we make a simple experiment ... 
        \item Factor 2: The distribution shift of the final detection scores due to the same reasons affects the accuracy of the downstream task. To demonstrate this, we make a simple experiment ... 
    \end{itemize}
    Therefore, calibrating these distributions is expected to abstract away the detector design from both the postprocessing and the downstream task.
    \item \textit{Hypothesis 2: Calibration enables different types of detectors to be ensembled (stacked) properly for the sake of better accuracy in terms of both AP and the downstream task accuracy.} Following from the previous hypothesis, the distribution difference (miscalibration) across the scores of the different types of detectors makes it non-trivial to obtain a high-performing ensemble model from them. Properly calibrating all detectors in an ensemble is expected to increase their accuracy. To demonstrate this, we make a simple experiment ...
\end{itemize}

}


